An Efficient NAS-based Approach for Handling Imbalanced Datasets

Class imbalance is a common issue in real-world data distributions, negatively impacting the training of accurate classifiers. Traditional approaches to mitigate this problem fall into three main categories: class re-balancing, information transfer, and representation learning. This paper introduces a novel approach to enhance performance on long-tailed datasets by optimizing the backbone architecture through neural architecture search (NAS). Our research shows that an architecture's accuracy on a balanced dataset does not reliably predict its performance on imbalanced datasets. This necessitates a complete NAS run on long-tailed datasets, which can be computationally expensive. To address this computational challenge, we focus on existing work, called IMB-NAS, which proposes efficiently adapting a NAS super-network trained on a balanced source dataset to an imbalanced target dataset. A detailed description of the fundamental techniques for IMB-NAS is provided in this paper, including NAS and architecture transfer. Among various adaptation strategies, we find that the most effective approach is to retrain the linear classification head with reweighted loss while keeping the backbone NAS super-network trained on the balanced source dataset frozen. Finally, we conducted a series of experiments on the imbalanced CIFAR dataset for performance evaluation. Our conclusions are the same as those proposed in the IMB-NAS paper.

==> content/convergence.tex <==
In this section, we analyze the convergence bound of the aggregated models on clients in Ferrari after $T$ training epochs with the theories of domain adaptation \cite{ben2006analysis}.  
Considering the pesonalized federated learning with $K$ clients, each client $i$ $(\forall i \in \{1,2,\dots,K \} )$ holds the local domain $\mathcal{T}_i : \langle \mathcal{D} _i ,f_i^*\rangle$ with $\mathcal{D} _i =\mathcal{D}_i^s\bigcup\mathcal{D}_i^u $, where $\mathcal{D}_i^s$ and 
$\mathcal{D}_i^u$ are labeled and unlabeled smaples from personalized data distribution $\mathcal{P} _{X,Y}^i$ and its marginal distribution $\mathcal{P}_X^i$, respectively.
$f_i^*$ denotes the labeling function that maps data $x \backsim \mathcal{P} _X^i$ to its true label. 
We treat client $i$ as the target domain and its received models from other similar clients as the source domains. 
Then the source domains can be defined as $\mathcal{T}_j : \langle \mathcal{D} _j ,f_j^*\rangle_{ \vert {j\in  {[ N_i ]}}} $, where $\mathcal{D} _j$ is the local data of migrating client $j$. 
%and $N_i$ denotes the number of other clients' models will be migrated to client $i$. 

%To analyze the feasibility of the proposed mechanism, we prove that ESFL can achieve a linear speedup convergence rate.
% \bluenote{For the sake of analysis}, we make the following three assumptions as suggested in \cite{wang2019adaptive, yang2020achieving, haddadpour2021federated, basu2020qsparse}.

% $\epsilon _i(h)       \epsilon _j(h)    \frac{1}{2}d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P} _X^i,\mathcal{P} _X^j)      
%                \lambda _j                   \frac{1}{N_i}\sum _{j=1}^{N_i}          \mathcal{T}_i          $

% $4\sqrt{\frac{ 2d\log 2em^* +\log{\frac{4M}{\mu }}}{m^*}}$
% $\hat{d}_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{D} _i,\mathcal{D} _j)$

% These assumptions are standard in non-convex optimization problems (\eg, training deep neural networks) and
% \bluenote{commonly used} in the analysis of FL with model compression \cite{haddadpour2021federated, basu2020qsparse}.

% In order to facilitate the proof of Theorem \ref{theorem}, we present several important lemmas as follows.
% The proofs of the lemmas mainly refer to Lemmas D.1-D.3 in \cite{haddadpour2021federated}, which can be directly applied to support our lemmas with little modification. 
% Therefore, to better highlight our main contributions, we omit the detailed proofs.
%we omit the proofs of these lemmas due to the limited space}.
% Due to the limited space, we omit the proof of these lemmas, and the detailed proof can be found in \cite{yang2020achieving}.
\begin{lemma}\cite{blitzer2007Learning}\label{lemma1}
    Suppose source domain $\mathcal{T}_j $ consists of $m$ labeled samples. $\mathcal{H}$ denotes a hypothesis space of VC-dimension $d$ \cite{sewell2008vc}. 
    Then $\forall \mu \in (0,1)$, with probability at least $1-\mu$ , $\forall h \in \mathcal{H}$: 
\begin{equation}
    \epsilon _i(h) \leq \epsilon _j(h)+ \frac{1}{2}d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P} _X^i,\mathcal{P} _X^j ) +\lambda _j
\end{equation}
where $\lambda _j=\min_{h \in \mathcal{H}}\epsilon _i(h) +  \epsilon _j(h)  $ and $\epsilon _i(h)$ denotes the ideal risk of hypothesis $h$ on domain 
$\mathcal{T}_i$. Additionally, $d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P} _X^i,\mathcal{P} _X^j)$ is the divergence of the data distributions $\mathcal{P} _X^i$ and $\mathcal{P} _X^j$
measured in a symmetric difference hypothesis space. 
\end{lemma}

Lemma \ref{lemma1} implies that the performance of hypothesis $h$ on distribution $\mathcal{P} _X^i$, assuming it behaves well on the marginal distribution of client $j$ (\ie, $\mathcal{P} _X^j$), is contingent on the divergence between the distributions $\mathcal{P} _X^i$ and $\mathcal{P} _X^j$ (\ie, $d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P} _X^i,\mathcal{P} _X^j)$). 
In other words, when the divergence between the two datasets is small, a model that performs well on one dataset can also achieve excellent performance on the other dataset.
    
\begin{corollary}\label{cly}
    For each client $i$, let $\hat{h}= \frac{1}{N_i}\sum _{j=1}^{N_i}h_j$ denote the aggregated hypothesis of migrated models, including $h_i$ itself. 
    Then $\forall \mu \in (0,1)$, with probability at least $1-\mu$, $\forall h \in \mathcal{H}$:
\begin{equation}
    \epsilon _i(\hat{h}) \leq \frac{1}{{N_i}}\sum _{j=1}^{N_i}\epsilon _j(h_j)+\frac{1}{2N_i}\sum _{j=1}^{N_i}d_{
        \mathcal{H} \Delta \mathcal{H}}(\mathcal{P} _X^i,\mathcal{P} _X^j+2\lambda _j  ) 
\end{equation}
\end{corollary}

Based on Lemma \ref{lemma1}, given the source client $j$ and the target client $i$, $\forall  \frac{\mu }{{N_i}} > 0 $, with probability $1- \frac{\mu }{{N_i}}$, we have:
\begin{equation}
    \epsilon _i(h_j) \leq \epsilon _j(h_j)+ \frac{1}{2}d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P} _X^i,\mathcal{P} _X^j ) +\lambda _j
\end{equation}
The convexity of empirical estimation ensures the validity of the Jenson inequality \cite{zhu2008jensen}:
\begin{equation}
    \epsilon _i(\hat{h}) = \epsilon _i(\frac{1}{{N_i}}\sum _{j=1}^{N_i} h_j) \leq \frac{1}{{N_i}}\sum _{j=1}^{N_i}\epsilon _i(h_j)
\end{equation}

Therefore, let $d^{'}=\frac{1}{2}d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P} _X^i,\mathcal{P} _X^j)$, $Pr\{ \cdot \} $ denote the probability. Then we have
%\vspace{-0.5cm}
\vspace{-0.3cm}
\begin{align}
    &Pr\{ \epsilon _i(\hat{h}) > \frac{1}{{N_i}}\sum _{j=1}^{N_i}(\epsilon _j(h_j)+d^{'}+ \lambda _j ) \}  \notag\\
    &\leq Pr\{ \frac{1}{{N_i}}\sum _{j=1}^{N_i}\epsilon _i(h_j) >\frac{1}{{N_i}}\sum _{j=1}^{N_i}(\epsilon _j(h_j)+ d^{'}+ \lambda _j \}  \notag\\
    &\leq Pr\{ \bigvee _{j\in[ N_i] } \epsilon _i(h_j) > \epsilon _j(h_j)+d^{'}+ \lambda _j \}  \leq \sum _{j=1}^{N_i} \frac{\mu }{{N_i}}=\mu 
\end{align}




% \vspace{-0.3cm}
% \begin{align}
%     &-\mathbb{E}\left[\left\langle\nabla F(\boldsymbol{w}^{h}), \mathbf{g}^{h}\right\rangle\right] \notag\\
%     &\leq \frac{\eta}{2 N}\sum_{i=1}^{N} \sum_{i=0}^{\tau-1}\left[-\|\nabla F(\boldsymbol{w}^{h})\|^{2}-\|\nabla F_i(\boldsymbol{w}_{i}^{(i, h)})\|^{2}\right]  \notag\\
%     &+\frac{\eta}{2 N}\sum_{i=1}^{N} \sum_{i=0}^{\tau-1} \left[L^{2}\|\boldsymbol{w}^{h}-\boldsymbol{w}_{i}^{(i, h)}\|^{2}\right]
% \end{align}


Combining these assumptions and lemmas, we can obtain the following theorem about the convergence bound.
%Due to the space limitation, the detailed proof is omitted here.
\begin{theorem}\label{theorem}
    For the FSSL system with K clients, $N_i$ clients are selected to build the aggregated hypothesis $\hat{h}= \frac{1}{{N_i}}\sum _{j=1}^{N_i}h_j$ for client $i$. 
There are two generalization bounds for applying $\hat{h}$ to domain  $\mathcal{T}_k$ \cite{shi2022uncertainty}:
    \begin{align}\label{convergance1}
        &\epsilon _i(\hat{h}) \leq \frac{1}{{N_i}}\sum _{j=1}^{N_i}(\epsilon _j(h_j)+ \frac{1}{2}\hat{d}_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{D} _i,\mathcal{D}_j)+ \lambda _j ) \notag\\
        &+4\sqrt{\frac{ 2d\log 2em^* +\log{\frac{4N_i}{\mu }}}{m^*}} \notag\\ 
    \end{align}
    \begin{align}\label{convergance2}
        &\epsilon _i(\hat{h})  \leq \frac{1}{{N_i}}\sum _{j=1}^{N_i}\hat{\epsilon _i}(h_j)+\sqrt{\frac{ 4d\log {\frac{2em}{d}} +\log{\frac{4N_i}{\mu }}}{m}}
    \end{align}
    where $\hat{\epsilon _i}$ and  $\hat{\epsilon _j}$ are empirical risks on domain  $\mathcal{T}_i$ and $\mathcal{T}_j$, respectively.
    $m$ denotes the sample size of labeled data. e is the natural constant and $m^*$ is the size of $\mathcal{D}_i$ and $\mathcal{D}_j $. 
    $\hat{d}_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{D}_i,\mathcal{D}_j)$ is the empirical estimate of $d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P} _X^i,\mathcal{P} _X^j)$.
\end{theorem}

% \rednote{Due to the smoothness in Assumption \ref{Lip}, taking expectation of $F\left(\boldsymbol{w}^{h+1}\right)$ and $F\left(\boldsymbol{w}^{h}\right)$
% over the randomness in the $h$-th epoch, then proce eding to use Lemma \ref{lemma1}, Lemma \ref{lemma2} and Lemma \ref{lemma3}, we have}
% Due to the smoothness in Assumption \ref{Lip} on global loss function,
% %by using unbiased estimate stochastic 
% by using the gradient $\mathbf{g}^{h}$ in Eq. \eqref{equ:gradient}, we have

%qikan
% \begin{proof}
%     Based on Vapnik-Chervonenkis theory:
% \begin{equation}
% %    \begin{small}
%     \begin{aligned}\label{proof}
%         &\epsilon _i(h_j) \leq \hat{\epsilon _i}(h_j)+\sqrt{\frac{ 4d\log {\frac{2em}{d}} +\log{\frac{4}{\mu }}}{m}}
%     \end{aligned}
% %    \end{small}
% \end{equation}


% Futher,we adopt the derivation in \cite{blitzer2007Learning}:

% \begin{equation}
%     %    \begin{small}
%     \begin{aligned}
%         &\frac{1}{2}d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P} _X^i,\mathcal{P} _X^j) \leq \frac{1}{2}\hat{d}_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{D} _i,\mathcal{D} _j)\\
%         &+4\sqrt{\frac{ 2d\log (2em^*) +\log{\frac{4N_i}{\mu }}}{m^*}}\\
%     \end{aligned}
%     %    \end{small}
% \end{equation}
% According to Theorem  1:
% \begin{equation}
%     %    \begin{small}
%     \begin{aligned}
%         &\epsilon _i(\hat{h}) \leq \frac{1}{{N_i}}\sum _{j=1}^{N_i}\epsilon _i(h_j) \\
%         &\leq \frac{1}{{N_i}}\sum _{j=1}^{N_i}\epsilon _j(h_j)+\frac{1}{2N_i}\sum _{j=1}^{N_i}(d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P} _X^i,\mathcal{P} _X^j+2\lambda _j  ). \\
%     \end{aligned}
%     %    \end{small}
% \end{equation}
% Thus, one can derive
% \begin{equation}
%     \begin{aligned}
%         &\epsilon _i(\hat{h}) \leq \frac{1}{{N_i}}\sum _{j=1}^{N_i}\epsilon _i(h_j) \\
%         &\leq \frac{1}{{N_i}}\sum _{j=1}^{N_i}\epsilon _j(h_j)+\frac{1}{2N_i}\sum _{j=1}^{N_i}(d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P} _X^i,\mathcal{P} _X^j+2\lambda _j  ). \\
%         &\leq \frac{1}{{N_i}}\sum _{j=1}^{N_i}(\epsilon _j(h_j)+\frac{1}{2}\hat{d}_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{D} _i,\mathcal{D} _j)+ \lambda _j) \\
%         &+4\sqrt{\frac{ 2d\log 2em^* +\log{\frac{4N_i}{\mu }}}{m^*}}
%     \end{aligned}
% \end{equation}

% and
% \begin{equation}
%     \begin{aligned}
%         &\epsilon _i(\hat{h})  \leq \frac{1}{{N_i}}\sum _{j=1}^{N_i} \epsilon _i(h_j) \\
%         &\leq \frac{1}{{N_i}}\sum _{j=1}^{N_i}\hat{\epsilon _i}(h_j)+\sqrt{\frac{ 4d\log {\frac{2em}{d}} +\log{\frac{4N_i}{\mu }}}{m}}
%     \end{aligned}
% \end{equation}
% \end{proof}

% Due to space limitation, we omit the detailed proof here.
% Therefore, the formulations \ref{} and \ref{} represent the two bounds in Theorem 1.
Eqs. \eqref{convergance1} and \eqref{convergance2} are two generalization bounds for the aggregated hypothesis. 
When the labeled dataset is large, the generalization
risk is bound by $ O \left(  \sqrt{\frac{d}{m}\log{\frac{m}{d}}-\frac{1}{m}\log{(\mu)}}\right)\approx 0 $ for Eq. \eqref{convergance2}, thus the empirical risk $\hat{\epsilon _i}(h_j)$ is available to measure the generalization 
bound of $\hat{h}$. When $m$ is small (close to zero), then the second term of Eq. \eqref{convergance2} could be too large thus diminishing the impact of empirical risk. Therefore, Eq. \eqref{convergance1}
is more appropriate for evaluating the generalization bound. 
These intuitions urge us to design a metric that quantifies the data relationship between heterogeneous clients, which is introduced in \S\ref{Generate Similarity-based Ranking}.
%\begin{equation}
%%    \begin{small}
%    \begin{aligned}
%    \notag&\mathbb{E}\left[\mathbb{E}_{\operatorname{top}_{i}}\left[F\left(\boldsymbol{w}^{h+1}\right)-F\left(\boldsymbol{w}^{h}\right)\right]\right] \\
%    &\leq \frac{\alpha \eta}{2 N}\sum_{i=1}^{N} \sum_{i=0}^{\tau-1} \left[-\left\|\nabla F\left(\boldsymbol{w}^{h}\right)\right\|_{2}^{2}-\left\|\mathbf{g}_{i}^{(i, h)}\right\|_{2}^{2}\right]\\
%    &+\frac{\alpha \eta}{2 N} \sum_{i=1}^{N} \sum_{i=0}^{\tau-1} \left[L^{2} \eta^{2} \sum_{c=0}^{\tau-1}\left[\tau\left\|\mathbf{g}_{i}^{(i, h)}\right\|_{2}^{2}+\mu^{2}\right]\right]\\
%    &+\frac{\left(2-\gamma\right) \alpha^{2} L}{2}\left[\frac{\eta^{2} \tau}{N} \sum_{i=1}^{N} \sum_{i=0}^{\tau-1}\left\|\mathbf{g}_{i}^{(i, h)}\right\|^{2}+\frac{\tau \eta^{2} \mu^{2}}{N}\right] \\
%    &\stackrel{\circled{1}}{\leq} \frac{\alpha \eta}{2 N} \sum_{i=1}^{N} \sum_{i=0}^{\tau-1}\left[-\left\|\nabla F\left(\boldsymbol{w}^{h}\right)\right\|_{2}^{2}-\left\|\mathbf{g}_{i}^{(i, h)}\right\|_{2}^{2}\right]\\
%    &+\frac{\alpha \eta}{2 N}\sum_{i=1}^{N} \sum_{i=0}^{\tau-1}\left[\tau L^{2} \eta^{2}\left[\tau\left\|\mathbf{g}_{i}^{(i, h)}\right\|_{2}^{2}+\mu^{2}\right]\right] \\
%    &+\frac{\left(2-\gamma\right) \alpha^{2} L}{2}\left[\frac{\eta^{2} \tau}{N} \sum_{i=1}^{N} \sum_{i=0}^{\tau-1}\left\|\mathbf{g}_{i}^{(i, h)}\right\|^{2}+\frac{\tau \eta^{2} \mu^{2}}{N}\right] \\
%    &=-\eta \alpha \frac{\tau}{2}\left\|\nabla F\left(\boldsymbol{w}^{h}\right)\right\|_{2}^{2} \\
%    &-\left(1-\tau^2 L^{2} \eta^{2} -\left(2-\gamma\right) \eta \alpha L \tau\right) \frac{\eta \gamma}{2 N} \sum_{i=1}^{N} \sum_{i=0}^{\tau-1}\left\|\mathbf{g}_{i}^{(i, h)}\right\|^{2}\\
%    &+\frac{L \tau \alpha \eta^{2}}{2 N}\left(N L \tau \eta+\alpha\left(2-\gamma\right)\right) \mu^{2} \\
%    &\stackrel{\circled{2}}{\leq}-\eta \alpha \frac{\tau}{2}\left\|\nabla F\left(\boldsymbol{w}^{h}\right)\right\|_{2}^{2}+\frac{L \tau \alpha \eta^{2}}{2 N}\left(N L \tau \eta+\alpha\left(2-\gamma\right)\right) \mu^{2}
%    \end{aligned}
%%    \end{small}
%\end{equation}
% \begin{equation}
% %    \begin{small}
% \begin{aligned}
% \notag&\mathbb{E}\left[\mathbb{E}_{\operatorname{top}_{i}}\left[F(\boldsymbol{w}^{h+1})-F(\boldsymbol{w}^{h})\right]\right] \\
% &\leq \frac{\alpha \eta}{2 N}\sum_{i=1}^{N} \sum_{i=0}^{\tau-1} \left[-\|\nabla F(\boldsymbol{w}^{h})\|^{2}-\|\mathbf{g}_{i}^{(i, h)}\|^{2}\right]\\
% &+\frac{\alpha \eta}{2 N} \sum_{i=1}^{N} \sum_{i=0}^{\tau-1} \left[L^{2} \eta^{2} \sum_{c=0}^{\tau-1}\left[\tau\|\mathbf{g}_{i}^{(i, h)}\|^{2}+\mu^{2}\right]\right]\\
% &+\frac{(2-\gamma) \alpha^{2} L}{2}\left[\frac{\eta^{2} \tau}{N} \sum_{i=1}^{N} \sum_{i=0}^{\tau-1}\|\mathbf{g}_{i}^{(i, h)}\|^{2}+\frac{\tau \eta^{2} \mu^{2}}{N}\right] \\
% &\stackrel{\circled{1}}{\leq} \frac{\alpha \eta}{2 N} \sum_{i=1}^{N} \sum_{i=0}^{\tau-1}\left[-\|\nabla F(\boldsymbol{w}^{h})\|^{2}-\|\mathbf{g}_{i}^{(i, h)}\|^{2}\right]\\
% &+\frac{\alpha \eta}{2 N}\sum_{i=1}^{N} \sum_{i=0}^{\tau-1}\left[\tau L^{2} \eta^{2}\left[\tau\|\mathbf{g}_{i}^{(i, h)}\|^{2}+\mu^{2}\right]\right] \\
% &+\frac{(2-\gamma) \alpha^{2} L}{2}\left[\frac{\eta^{2} \tau}{N} \sum_{i=1}^{N} \sum_{i=0}^{\tau-1}\|\mathbf{g}_{i}^{(i, h)}\|^{2}+\frac{\tau \eta^{2} \mu^{2}}{N}\right] \\
% &=-\eta \alpha \frac{\tau}{2}\|\nabla F(\boldsymbol{w}^{h})\|^{2} \\
% &-\left(1-\tau^2 L^{2} \eta^{2} -(2-\gamma) \eta \alpha L \tau\right) \frac{\eta \gamma}{2 N} \sum_{i=1}^{N} \sum_{i=0}^{\tau-1}\|\mathbf{g}_{i}^{(i, h)}\|^{2}\\
% &+\frac{L \tau \alpha \eta^{2}}{2 N}\left(N L \tau \eta+\alpha(2-\gamma)\right) \mu^{2} \\
% &\stackrel{\circled{2}}{\leq}-\eta \alpha \frac{\tau}{2}\|\nabla F(\boldsymbol{w}^{h})\|^{2}+\frac{L \tau \alpha \eta^{2}}{2 N}\left(N L \tau \eta+\alpha(2-\gamma)\right) \mu^{2}
% \end{aligned}
% %    \end{small}
% \end{equation}


% \begin{small}
% \begin{align}
%     &\frac{1}{H} \sum_{h=0}^{H-1}\left\|\nabla F\left(\boldsymbol{w}^{h}\right)\right\|_{2}^{2} \notag\\ 
%     \notag&\leq \frac{2\left(F\left(\boldsymbol{w}^{0}\right)-F\left(\boldsymbol{w}^{*}\right)\right)}{\eta \alpha \tau H}
%     +\frac{\operatorname{L\eta} \alpha \left(2-\gamma\right)}{N} \mu^{2}+L^{2} \eta^{2} \tau \mu^{2}
% \end{align}
% \end{small}

% On basis of Theorem \ref{theorem}, we can specify $\eta \alpha=\mathcal{O}(\frac{\sqrt{N}}{\sqrt{H \tau}})$ to achieve a linear speedup convergence rate, and further obtain the following convergence bound for our FedLamp with proper decisions of global aggregation weight $\frac{\alpha}{N}$ and local learning rate $\eta$.
% \begin{corollary}\label{cly}
%     Let $\eta=c_1\frac{\gamma}{\sqrt{H} \tau L}$ and $\alpha=c_2\sqrt{\tau N}$, where $c_1$ and $c_2$ are constant coefficients, then the convergence rate can be transformed as:
%     %\begin{small}
%     \begin{align}
%         &\frac{1}{H} \sum_{h=0}^{H-1}\|\nabla F\left(\boldsymbol{w}^{h}\right)\|^{2} \notag\\ 
%         &\leq \frac{2 L \left(F(\boldsymbol{w}^{0})-F(\boldsymbol{w}^{*})\right)}{c_1 c_2\gamma\sqrt{\tau H N}}
%         +\frac{c_1 c_2 \gamma (2-\gamma)\mu^{2} }{\sqrt{\tau H N}} \notag\\
%         &+ \frac{c_1^2 \gamma^2 \mu^2}{H \tau}
%     \end{align}
%     %\end{small}
% \end{corollary}

% %As the compression ratio $q \le \gamma \le 1$, which $q$ is a constant, we can achieve a linear speed up convergence rate $\mathcal{O}\left(\frac{1}{\sqrt{\tau H N}}\right)$.
% With Corollary \ref{cly}, FedLamp can achieve a linear speedup of convergence rate $\mathcal{O}(\frac{1}{\sqrt{\tau H N}})$ as many previous works \cite{wang2019adaptive, yang2020achieving, haddadpour2021federated}, which indicates that FedLamp can contribute to saving resource consumption while still maintaining the similar convergence performance.
% Upon the setting $\alpha=c_2\sqrt{\tau N}$, we can formulate a rule to assign the global aggregation weight $\frac{\alpha_i^h}{N}$ for worker $i$ at round $h$, where $\alpha_i^h$ is expressed as follows:
% %\begin{equation}
% %    \alpha_i^h=\frac{N\tau_i^h}{\sqrt{\sum_{i=1}^N{\tau_i^h}}}
% %\end{equation}
% \begin{equation}
% \alpha_i^h=c_2\sqrt{\tau_i^h N}
% \end{equation}
% which indicates that a model trained with larger local updating frequency will be assigned with a larger global aggregation weight, so as to improve overall training efficiency. 
% Since $\sum_{i=1}^N \frac{\alpha_i^h}{N}=1$, we can obtain that $c_2=\frac{\sqrt{N}}{\sum_{i=1}^N\sqrt{\tau_i^h}}$.

% Given the local learning rate $\eta=c_1\frac{\gamma}{\sqrt{H} \tau L}$, we can formulate a scaling rule to guide the setting of model compression ratios for different workers with respect to their local updating frequencies as follows:
% \begin{equation}
% \frac{\gamma_i^h}{\tau_i^h} = v
% \end{equation}
% where $v=\frac{\eta L \sqrt{H}}{c_1}$ is a constant indicating that model compression ratio of worker is proportional to its local updating frequency.
% %, which indicates that models updated with more iterations of local updating will be assigned with larger compression ratios.
% Then the local updating completion time (including
% computing time and communication time) at the $h$-th communication round on worker $i$ can be rewritten as:
% \begin{equation}
% t_i^h=\tau_i^h (\mu_i^h+v \cdot \beta_i^h) 
% \end{equation}
% Considering the above analysis, we can solve the problem in Eq. (\ref{problem}) by determining the local updating frequencies and model compression ratios for workers upon the computing time $\mu_i^h$ and communication time $\beta_i^h$, which will be elaborated in Section \ref{sec:alg}.

%We can give the problem formulation later with the relationship between the number of local iterations and the compression ratio.

==> content/prelim.tex <==
In this section, we first introduce the sequential recommendation task and then present a brief review of the compression method used in our current work to help understand the new contributions.

\subsection{ Problem Formulation }
In the setting of sequential recommendation, let a set of $n$ users $\mathcal{U}$ interact independently with a set of $m$ items $\mathcal{I}$, and each $i \in \mathcal{I}$ has features $\mathrm{F}_i \in \mathbb{R}^d$, where $d$ is the number of dimensions. 
For each user $u \in \mathcal{U}$, it has a sequential interaction with items $S_u=\left\{i_1, i_2, \ldots i_w\right\}$, where $w$ denotes the length of the sequence. 
% Note that we use numbered subscripts for items mainly to indicate their orders in a sequence. 
The sequential recommendation aims to predict the next item of $ i_{w+1} $ that matches the user's preferences, given his historical interactions $S_u$.
The user's preferences can be inferred from our well-designed GNN model. 


\subsection{Embedding Compression}
Quantization, as an effective compression method, can compress a network by replacing the 32-bit full-precision weights with their lower-bit counterparts without changing the network architecture. Specifically, for $m$ bit quantization, the set of the quantized values can be denoted as $\mathbb{S}=\left\{b_0, b_1, \ldots, b_k\right\}$, where $k=2^m-1$.
In the uniform symmetric quantization, the step size $\Delta=b_t-b_{t-1}$ remains the same for any $t \in[1, k]$, and $b_0=-2^{m-1} \Delta, b_k=\left(2^{m-1}-1\right) \Delta$.
In this paper, we adopt uniform symmetric quantization on the item embeddings, which is usually more hardware-friendly than the non-uniform quantization, and the quantized values are uniformly distributed.
Specially, given the step size $\Delta$ and the bit width $m$, a full-precision weight $w$ is quantized into $\hat{w} \in \mathbb{S}$, which is represented by the multiplication of the step size $\Delta$ and an integer $\tilde{w}$ :

\begin{equation}
    \begin{gathered}
\tilde{w}=R\left(\operatorname{clip}\left(w / \Delta,-2^{m-1}, 2^{m-1}-1\right)\right), \\
\end{gathered}
\end{equation}

\begin{equation}
    \begin{gathered}
    \hat{w}=Q(w)=\Delta \times \tilde{w},
    \end{gathered}
\end{equation}



where $\operatorname{clip}(v, n, p)$ returns $v$ with values below $n$ set to $n$ and values above $p$ set to $p$ and $R(v)$ rounds $v$ to an adjacent integer. 
% There are generally two kinds of rounding functions:
We allow two rounding options: deterministic rounding and stochastic rounding.
If deterministic rounding is used, a floating-point value is rounded to its nearest integer:
\begin{equation}
\begin{gathered}
    R_D(x)= \begin{cases}\lfloor x\rfloor & \text { if } x-\lfloor x\rfloor<0.5, \\ \lfloor x\rfloor+1 & \text { otherwise. }\end{cases}
\end{gathered}
\end{equation}



If stochastic rounding is used, a floating-point value is rounded to its two adjacent integers with a probability distribution:
\begin{equation}
\begin{gathered}
R_S(x)=\left\{\begin{array}{lll}
\lfloor x\rfloor & \text { w.p. } & \lfloor x\rfloor+1-x \\
\lfloor x\rfloor+1 & \text { w.p. } & \quad x-\lfloor x\rfloor .
\end{array}\right.
\end{gathered}
\end{equation}


\subsection{System Overview}\label{sec-sys-overview}
xxx follows the typical FL client-server architecture, as illustrated in Section \ref{sec_introduction}.
In this setup, each client holds a single user's interaction data and trains a lightweight recommender model.
A client maintains an embedding model and a recommender model, while the PS keeps the aggregated embedding model and recommender model. 
The detailed
design of the client and server are presented in Sections \ref{sec:design}.

